Tensor Regression Meets Gaussian Processes

Low-rank tensor regression, a new model class that learns high-order correlation from data, has recently received considerable attention. At the same time, Gaussian processes (GP) are well-studied machine learning models for structure learning. In this paper, we demonstrate interesting connections between the two, especially for multi-way data analysis. We show that low-rank tensor regression is essentially learning a multi-linear kernel in Gaussian processes, and the low-rank assumption translates to the constrained Bayesian inference problem. We prove the oracle inequality and derive the average case learning curve for the equivalent GP model. Our finding implies that low-rank tensor regression, though empirically successful, is highly dependent on the eigenvalues of covariance functions as well as variable correlations.

==> application.tex <==
% elaborate the applications

\paragraph{Multi-linear Multi-task learning}


\paragraph{Spatio-temporal Forecasting}

==> preliminary.tex <==
Across the paper, we use calligraphy font for tensors, such as $\T{X},\T{Y}$; bold uppercase letters for matrices, such as $\M{X},\M{Y}$; and bold lowercase letters for vectors, such as $\V{x},\V{y}$. In the paper, we use three-order tensors for the ease of explanation. 

\textbf{Tensor Unfolding}
Each dimension of a tensor is a mode. An n-mode unfolding along mode $n$ transforms a tensor $\T{W} $ into a matrix $\T{W}_{(n)}$ by treating $n$ as the first mode of the matrix and cyclically concatenating other modes. 
%It is also known as tensor matricization. 
%Multiple mode unfolding is not considered in this paper \ryedit{We only consider single mode unfolding or Remove this sentence}.

\textbf{N-Mode Product}
The n-mode product between tensor $\T{W}$ and matrix $\M{U}$ on mode $n$ is represented as $\T{W}\times_n \M{U}$ and is defined as $(\T{W}\times_n\M{U})_{(n)} = \M{U} \T{W}_{(n)}$ .

% \textbf{reduced QR decomposition}
% QR decomposition factorize the matrix $W\in \R^{m\times n}$ into a product of a unitary matrix $Q \in \R^{m\times m}$ and an upper triangular matrix $R \in \R^{m\times n}$, $m \geq n$. the reduced QR composition of order $r$ consists of the first $r$ columns of $Q$ and top $r$ rows of R.

\textbf{Tucker Decomposition}
Tucker decomposition factorizes a tensor $\T{W}\in \R^{D_1 \times \cdots \times D_n}$ into 
$\T{W} = \skt \times_1 \M{U}_1 \cdots \times_n \M{U}_n$, where $\{\M{U}_n \in \R^{R_n \times D_n}\}$ are all unitary matrices and the core tensor satisfies that $\skt_{(n)} \in \R^{R_1\times \cdots \times R_n}$ is row-wise orthogonal for all $n=1,2,\dots,N$. 

%\cite{tucker1966some}

==> relate.tex <==
Multi-task feature learning \cite{evgeniou2007multi} explores task relatedness to improve the performance when learning multiple tasks simultaneously.  Tensor regression \cite{romera2013multilinear} further exploits the  multi-directional task relatedness and formulates a regression problem with tensor structural constraint. Many  algorithms have been proposed to solve the problem. For instance, \cite{wimalawarne2014multitask} improves upon the convex formulation of \cite{romera2013multilinear} and studies a novel schatten norm regularizer. \cite{yu2014fast, yu2016learning} employ the non-convex optimization techniques and achieve further acceleration. However, all of them rely on deterministic models and cannot  explicitly express uncertainty. 

Lately, Bayesian tensor regression has been investigated, mostly in statistics community. \cite{hoff2015multilinear} chooses  a Gaussian-inverse Wishart prior  to model each factor in the parameter tensor separately. \cite{guhaniyogi2015bayesian} proposes a  multiway Dirichlet generalized double Pareto prior, in order to induce shrinkage across components. However, both models are parametric with limited flexibility, and the parameter inferences are hard to scale. Non-parametric models for multi-way data has been studied in \cite{chu2009probabilistic, xu2012infinite}



%\paragraph{Multi-task feature learning}
%From a probabilistic perspective, model $\V{y}_{t,i} \sim \T{N}(f_t(\V{x}_{t,i}), \sigma_t^2)$ with kernel matrix $\langle  f_t(\V{x}_{t,i}), f_s(\V{x}_{s,j}) \rangle  = \M{K}^f_{ts}k^x(\V{x}_{t,i}, \V{x}_{s,j})$. GP prior can be placed over the latent functions $ \V{f} \sim \text{GP}(\V{0},\V{\Sigma}) $ with $\M{\Sigma} = \M{K}^f \otimes \M{K}^x \in \R^{TD \times TD}$  \cite{bonilla2007multi}. The low-rank constraint is enforced through the low-rank structure in $\M{K}^f$.    

%
%More generally, placing prior (?) on $\text{vec}(\V{y}) \sim \T{N}(f(\V{x}_{i})) $ equivalent model $\text{vec}(\M{Y})  = (\M{X} \otimes \M{I}_T) \text{vec}(\M{W}) + \V{e} $. 

%$p(\M{\Sigma}, \M{W}) \propto |\M{\Sigma}| ^{-(L+1/2)}$

\paragraph{Tensor-variate regression}
Tensor-variate regression, or multi-linear multi-task learning \cite{romera2013multilinear} aims to solve weights with tensor structural  constraint. 
\begin{align}
\sum_{t =1}^T \sum_{i=1}^{n_t} \loss (\langle \V{x}_{t,i}, \V{w}_t \rangle ; \V{y}_{t,i} ) \quad \text{s.t.} \quad \text{rank}(\T{W}) \leq R
\label{eqn:multilinear}
\end{align}
where $\T{W}_{(1)}=   [\V{w}_1,\cdots, \V{w}_T]$. Suppose $\T{W}$ follows Tucker model, $\T{W} = \T{S} \times_1 \M{U}_1 \times_2 \M{U}_2 \times_3 \M{U}_3$. Equivalently, $\text{vec}(\T{W}) =  (\M{U}_1 \otimes \M{U}_2 \otimes \M{U}_3) \text{vec}(\T{S})$.



In tensor decomposition literature, let $\vt(\T{S}) \sim N(0,1)$, Tucker model can be represented as    $\text{vec}(\T{W}) \sim \T{N}(\M{0}, \M{\Sigma}\M{\Sigma}^\top + \sigma \M{I})$, where $\M{\Sigma} = \M{U}_3 \otimes \M{U}_2 \otimes \M{U}_1$ and $\sigma$ is the observation noise \cite{chu2009probabilistic}. 


\paragraph{Gaussian process regression}
Non-parametric methods, such as Gaussian process (GP) \cite{rasmussen2006gaussian} provides a flexible framework for structure discovery in complex data. Given  inputs $\M{X}= \{ \V{x}_i \in \R^D\}_{i=1}^N $ and outputs $\M{Y} = \{\V{y} \in \R \}_{i=1}^N$, Gaussian process model assumes: 
\begin{align}
 \V{y}_i = f(\V{x}_i) +  \epsilon,   \quad  f(\V{x}_i)  \sim \text{GP} (m_{\theta_m}, K_{\theta_K}),  \quad \epsilon \sim N(0, \sigma)
\label{eqn:gp}
	\end{align}
where $m_{\theta_m}$ is the mean function, and $K_{\theta_K}$ is the covariance function. Due to $\T{O}(N^3)$ runtime  and $\T{O}(N^2)$ space complexity, GP suffers from computation bottleneck. Many work try to  improve scalability by exploiting kernel structures, such as inducing point methods FITC \cite{snelson2005sparse}, kronecker product \cite{NIPS2014} or the two combined \cite{wilson2015kernel} \ryedit{Double check}.

